Lost in Moderation: How Commercial Content Moderation APIs Over- and Under-Moderate Group-Targeted Hate Speech and Linguistic Variations

Commercial content moderation APIs are marketed as scalable solutions to combat online hate speech. However, the reliance on these APIs risks both silencing legitimate speech, called over-moderation, and failing to protect online platforms from harmful speech, known as under-moderation. To assess such risks, this paper introduces a framework for auditing black-box NLP systems. Using the framework, we systematically evaluate five widely used commercial content moderation APIs. Analyzing five million queries based on four datasets, we find that APIs frequently rely on group identity terms, such as ``black'', to predict hate speech. While OpenAI's and Amazon's services perform slightly better, all providers under-moderate implicit hate speech, which uses codified messages, especially against LGBTQIA+ individuals. Simultaneously, they over-moderate counter-speech, reclaimed slurs and content related to Black, LGBTQIA+, Jewish, and Muslim people. We recommend that API providers offer better guidance on API implementation and threshold setting and more transparency on their APIs' limitations. Warning: This paper contains offensive and hateful terms and concepts. We have chosen to reproduce these terms for reasons of transparency.

==> latexmkrc.tex <==
$pdflatex = "latexdiff --exclude-textcmd=midrule,toprule,bottomrule Main_old.tex Main.tex  > main-d.tex; pdflatex %O  main-d"

==> tables.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccccccc|l}
\hline
Category     & \textbf{CS-FN} & \textbf{DE-FN} & \textbf{IMP} & \textbf{NE-FN} & \textbf{NOHATE} & \textbf{PAR} & \textbf{POS} & \textbf{SPELL} & \textbf{UNSURE} & \textbf{SUM} \\ 
\hline
GPT & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{177.26865671641792, 194.1044776119403, 255}{23\%} & \colorbox[RGB]{182.12686567164178, 197.91044776119404, 255}{22\%} & \colorbox[RGB]{240.42537313432837, 243.5820895522388, 255}{4\% \hspace{0.8mm}} & \colorbox[RGB]{201.55970149253733, 213.13432835820896, 255}{16\%} & \colorbox[RGB]{220.99253731343282, 228.3582089552239, 255}{10\%} & \colorbox[RGB]{245.28358208955223, 247.38805970149252, 255}{2\% \hspace{0.8mm}} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{191.84328358208955, 205.52238805970148, 255}{19\%} & 67 \\ 
Google & \colorbox[RGB]{237.73863636363637, 241.47727272727272, 255}{5\% \hspace{0.8mm}} & \colorbox[RGB]{176.0909090909091, 193.1818181818182, 255}{24\%} & \colorbox[RGB]{161.29545454545453, 181.59090909090907, 255}{28\%} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{227.875, 233.75, 255}{8\% \hspace{0.8mm}} & \colorbox[RGB]{225.4090909090909, 231.8181818181818, 255}{9\% \hspace{0.8mm}} & \colorbox[RGB]{220.47727272727272, 227.95454545454544, 255}{10\%} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{210.61363636363637, 220.22727272727272, 255}{13\%} & 132 \\ 
Microsoft & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{137.06521739130434, 162.6086956521739, 255}{36\%} & \colorbox[RGB]{141.7826086956522, 166.30434782608694, 255}{34\%} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{231.41304347826087, 236.52173913043478, 255}{7\% \hspace{0.8mm}} & \colorbox[RGB]{231.41304347826087, 236.52173913043478, 255}{7\% \hspace{0.8mm}} & \colorbox[RGB]{231.41304347826087, 236.52173913043478, 255}{7\% \hspace{0.8mm}} & \colorbox[RGB]{240.84782608695653, 243.91304347826087, 255}{4\% \hspace{0.8mm}} & \colorbox[RGB]{245.56521739130434, 247.6086956521739, 255}{2\% \hspace{0.8mm}} & 69 \\ 
Perspective & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{127.27215189873418, 154.9367088607595, 255}{39\%} & \colorbox[RGB]{164.35443037974684, 183.98734177215192, 255}{27\%} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{230.27848101265823, 235.63291139240505, 255}{7\% \hspace{0.8mm}} & \colorbox[RGB]{230.27848101265823, 235.63291139240505, 255}{7\% \hspace{0.8mm}} & \colorbox[RGB]{234.3987341772152, 238.86075949367088, 255}{6\% \hspace{0.8mm}} & \colorbox[RGB]{255.0, 255.0, 255}{0\% \hspace{0.8mm}} & \colorbox[RGB]{217.91772151898735, 225.9493670886076, 255}{11\%} & 79 \\ 
 \hline
\end{tabular}
\caption{Second Table with Integer Values}
\end{table}
